No Need to Lift a Finger Anymore? Assessing the Quality of Code Generation by ChatGPT

Large language models (LLMs) have demonstrated impressive capabilities across various NLP tasks. Additionally, LLMs are also highly valuable in supporting software engineering tasks, particularly in the field of code generation. Automatic code generation is a process of automatically generating source code or executable code based on given specifications or requirements, improving developer productivity. In this study, we perform a systematic empirical assessment to the quality of code generation using ChatGPT. We leverage 728 algorithm problems in five languages (i.e., C, C++, Java, Python, and JavaScript) and 18 CWEs with 54 code scenarios for the code generation task. Our evaluation encompasses a comprehensive analysis of code snippets generated by ChatGPT, focusing on three critical aspects: correctness, complexity, and security. We also specifically investigate ChatGPT's ability to engage in multi-round fixing process (i.e., ChatGPT's dialog ability) of facilitating code generation. By delving into the generated code and examining the experimental results, this work provides valuable insights into the performance of ChatGPT in tackling code generation tasks over the three critical aspects. Overall, our findings uncover potential issues and limitations that arise in the ChatGPT-based code generation and lay the groundwork for improving AI and LLM-based code generation techniques.

==> Sections/data.tex <==
\section{Data Availability}\label{sec:data}
The experimental scripts, results, and raw data are available at: \cite{artifact}.

==> Sections/temp.tex <==

\begin{table*}[ht]
\centering
\caption{Code-judged Result in C, C++, and Java Languages}
\renewcommand\arraystretch{1.3}
\scalebox{0.6}{\begin{tabular}{c|c|rrrrr|rrrrr|rrrrr} 
\toprule
\multirow{2}{*}{Period} & \multirow{2}{*}{Difficulty} & \multicolumn{5}{c}{C}   & \multicolumn{5}{c|}{~C++~} & \multicolumn{5}{c}{Java}          \\ 
\cline{3-17}
                        &                             & \multicolumn{1}{c}{A.}  & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{C.E.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c}{R.E.} & \multicolumn{1}{c}{A.} & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{C.E.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c|}{R.E.} & \multicolumn{1}{c}{A.} & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{C.E.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c}{R.E.} \\ 
\midrule
\multirow{4}{*}{Aft.}   & Hard                        & \percent[t]{0}{91}   & \percent[t]{57}{91}   & \percent[t]{25}{91}   & \percent[t]{2}{91}      & \percent[t]{7}{91}    & \percent[t]{0}{91}                    &   \percent[t]{57}{91}                &      \percent[t]{24}{91}                  &       \percent[t]{7}{91}               &         \percent[t]{3}{91}                 &  \percent[t]{0}{90}                     &    \percent[t]{64}{90}                    &     \percent[t]{16}{90}                   &   \percent[t]{5}{90}                        & \percent[t]{5}{90}                   \\
                        
                        
                        
                        & Medium                      & \percent[t]{10}{170}  & \percent[t]{77}{170}   & \percent[t]{49}{170}   & \percent[t]{12}{170}     & \percent[t]{22}{170}     &   \percent[t]{23}{172}                   &  \percent[t]{99}{172}                      &  \percent[t]{23}{172}                      & \percent[t]{12}{172}                         & \percent[t]{15}{172}                        &   \percent[t]{26}{172}                   &  \percent[t]{119}{172}                     &  \percent[t]{13}{172}                      &  \percent[t]{10}{172}                        &  \percent[t]{4}{172}                   \\


                        
                        & Easy                        & \percent[t]{44}{90}  & \percent[t]{33}{90}   & \percent[t]{9}{90}   & \percent[t]{0}{90}      & \percent[t]{4}{90}   &   \percent[t]{45}{88}                   &  \percent[t]{40}{88}                      &  \percent[t]{1}{88}                       &   \percent[t]{1}{88}                        &   \percent[t]{1}{88}                       & \percent[t]{45}{90}                     & \percent[t]{37}{90}                       & \percent[t]{4}{90}                        & \percent[t]{2}{90}                         & \percent[t]{2}{90}               \\ 
\cline{2-17}


                        & Total                       & \percent[t]{54}{351}  & \percent[t]{167}{351}  & \percent[t]{83}{351}   & \percent[t]{14}{351}     & \percent[t]{33}{351}    & \percent[t]{68}{351}                     & \percent[t]{196}{351}                      & \percent[t]{48}{351}                       & \percent[t]{20}{351}                         & \percent[t]{19}{351}                        & \percent[t]{71}{352}                     & \percent[t]{220}{352}                      & \percent[t]{33}{352}                       & \percent[t]{17}{352}                         & \percent[t]{11}{352}            \\ 

                        
\midrule




\multirow{4}{*}{Bef.}   & Hard                        & \percent[t]{17}{93}  & \percent[t]{36}{93}   & \percent[t]{31}{93}   & \percent[t]{3}{93}      & \percent[t]{6}{93}     & \percent[t]{40}{94}                     & \percent[t]{18}{94}                       & \percent[t]{30}{94}                       & \percent[t]{2}{94}                          & \percent[t]{4}{94}                         & \percent[t]{47}{89}                     & \percent[t]{24}{89}                       & \percent[t]{12}{89}                       & \percent[t]{2}{89}                          & \percent[t]{4}{89}                    \\




                        & Medium                      & \percent[t]{80}{172}  & \percent[t]{35}{172}   & \percent[t]{36}{172}   & \percent[t]{5}{172}      & \percent[t]{16}{172}     & \percent[t]{125}{177}                    & \percent[t]{25}{177}                       & \percent[t]{21}{177}                       & \percent[t]{0}{177}                          & \percent[t]{6}{177}                         & \percent[t]{136}{174}                    & \percent[t]{21}{174}                       & \percent[t]{8}{174}                        & \percent[t]{6}{174}                          & \percent[t]{3}{174}                     \\

                        
                        & Easy                        & \percent[t]{74}{97}  & \percent[t]{9}{97}    & \percent[t]{6}{97}    & \percent[t]{0}{97}      & \percent[t]{8}{97}   & \percent[t]{91}{102}                     & \percent[t]{7}{102}                        & \percent[t]{2}{102}                        & \percent[t]{1}{102}                          & \percent[t]{1}{102}                         & \percent[t]{95}{101}                     & \percent[t]{4}{101}                        & \percent[t]{2}{101}                        & \percent[t]{0}{101}                          & \percent[t]{0}{101}         \\ 
\cline{2-17}


                        & Total                       & \percent[t]{171}{362} & \percent[t]{80}{362}   & \percent[t]{73}{362}   & \percent[t]{8}{362}      & \percent[t]{30}{362}     & \percent[t]{256}{373}                    & \percent[t]{50}{373}                       & \percent[t]{53}{373}                       & \percent[t]{3}{373}                          & \percent[t]{11}{373}                        & \percent[t]{278}{364}                    & \percent[t]{49}{364}                       & \percent[t]{22}{364}                       & \percent[t]{8}{364}                          & \percent[t]{7}{364}                        \\ 

                        
\midrule
-                       & Total                       & \percent[t]{223}{713} & \percent[t]{247}{713}  & \percent[t]{156}{713}  & \percent[t]{22}{713}     & \percent[t]{63}{713}  & \percent[t]{324}{724}                    & \percent[t]{246}{724}                      & \percent[t]{101}{724}                      & \percent[t]{23}{724}                         & \percent[t]{30}{724}                        & \percent[t]{349}{716}                    & \percent[t]{269}{716}                      & \percent[t]{55}{716}                       & \percent[t]{25}{716}                         & \percent[t]{18}{716}         \\
\bottomrule
\end{tabular}}
\label{tab:generation-1}
\end{table*}



\begin{table*}[ht]
\centering
\caption{Code-judged Result in Python3 and JavaScript Languages}
\renewcommand\arraystretch{1.3}
\scalebox{0.6}{\begin{tabular}{c|c|rrrr|rrrr} 
\toprule
\multirow{2}{*}{Period} & \multirow{2}{*}{Difficulty}                                                                                                              & \multicolumn{4}{c|}{Python3}                                                                               & \multicolumn{4}{c}{JavaScript}                                                                             \\ 
\cline{3-10}
                        &                              & \multicolumn{1}{c}{A.} & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c|}{R.E.} & \multicolumn{1}{c}{A.} & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c}{R.E.}  \\ 
\midrule
\multirow{4}{*}{Aft.}   & Hard                 & \percent[t]{2}{91}                      & \percent[t]{73}{91}                       & \percent[t]{11}{91}                         & \percent[t]{5}{91}                         & \percent[t]{1}{91}                      & \percent[t]{76}{91}                       & \percent[t]{5}{91}                          & \percent[t]{9}{91}                        \\
                        & Medium                     &   \percent[t]{31}{171}                   &     \percent[t]{105}{171}                   &     \percent[t]{19}{171}                      &   \percent[t]{16}{171}                       &  \percent[t]{29}{171}                    &  \percent[t]{116}{171}                     &  \percent[t]{17}{171}                        &  \percent[t]{9}{171}                       \\
                        & Easy                      & \percent[t]{51}{89}                     & \percent[t]{31}{89}                       & \percent[t]{2}{89}                          & \percent[t]{5}{89}                         & \percent[t]{49}{89}                     &  \percent[t]{34}{89}                      & \percent[t]{1}{89}                          & \percent[t]{5}{89}                         \\ 
\cline{2-10}
                        & Total                                   &  \percent[t]{84}{351}                    & \percent[t]{209}{351}                      & \percent[t]{32}{351}                         & \percent[t]{26}{351}                        & \percent[t]{79}{351}                     & \percent[t]{226}{351}                      & \percent[t]{23}{351}                         & \percent[t]{23}{351}                        \\ 
\midrule



\multirow{4}{*}{Bef.}   & Hard                             & \percent[t]{41}{90}                     & \percent[t]{30}{90}                       & \percent[t]{8}{90}                          & \percent[t]{11}{90}                        & \percent[t]{38}{90}                     & \percent[t]{42}{90}                       & \percent[t]{2}{90}                          & \percent[t]{8}{90}                         \\
                        & Medium                         &  \percent[t]{136}{172}                   & \percent[t]{28}{172}                       & \percent[t]{2}{172}                          & \percent[t]{6}{172}                         & \percent[t]{136}{169}                    & \percent[t]{22}{169}                       & \percent[t]{3}{169}                          & \percent[t]{8}{169}                        \\
                        & Easy                                          & \percent[t]{95}{99}                     & \percent[t]{4}{99}                        & \percent[t]{0}{99}                          & \percent[t]{0}{99}                         & \percent[t]{94}{101}                     & \percent[t]{6}{101}                        & \percent[t]{0}{101}                          & \percent[t]{1}{101}                         \\ 
\cline{2-10}
                        & Total                       &  \percent[t]{272}{361}                   & \percent[t]{62}{361}                       & \percent[t]{10}{361}                          & \percent[t]{17}{361}                        & \percent[t]{268}{360}                    & \percent[t]{70}{360}                       & \percent[t]{5}{360}                          & \percent[t]{17}{360}                        \\ 
\midrule
-                       & Total                                        & \percent[t]{356}{712}                    & \percent[t]{271}{712}                      & \percent[t]{42}{712}                         & \percent[t]{43}{712}                        & \percent[t]{347}{711}                    &  \percent[t]{296}{711}                     &  \percent[t]{28}{711}                        &   \percent[t]{40}{711}                      \\
\bottomrule
\end{tabular}}
\label{tab:generation-2}
\end{table*}

==> Sections/temp2.tex <==
\begin{table*}[ht]
\centering
\caption{Code-judged result in C++, Java, Python3 and JavaScript languages}
\renewcommand\arraystretch{1.3}
\scalebox{0.66}{\begin{tabular}{c|c|rrrrr|rrrrr|rrrr|rrrr} 
\toprule
\multirow{2}{*}{Period} & \multirow{2}{*}{Difficulty} & \multicolumn{5}{c|}{~C++~}                                                                                                            & \multicolumn{5}{c|}{Java}                                                                                                             & \multicolumn{4}{c|}{Python3}                                                                               & \multicolumn{4}{c}{JavaScript}                                                                             \\ 
\cline{3-20}
                        &                             & \multicolumn{1}{c}{A.} & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{C.E.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c|}{R.E.} & \multicolumn{1}{c}{A.} & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{C.E.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c|}{R.E.} & \multicolumn{1}{c}{A.} & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c|}{R.E.} & \multicolumn{1}{c}{A.} & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c}{R.E.}  \\ 
\midrule
\multirow{4}{*}{Aft.}   & Hard                        & \percent[t]{0}{91}                    &   \percent[t]{57}{91}                &      \percent[t]{24}{91}                  &       \percent[t]{7}{91}               &         \percent[t]{3}{91}                 &  \percent[t]{0}{90}                     &    \percent[t]{64}{90}                    &     \percent[t]{16}{90}                   &   \percent[t]{5}{90}                        & \percent[t]{5}{90}                        & \percent[t]{2}{91}                      & \percent[t]{73}{91}                       & \percent[t]{11}{91}                         & \percent[t]{5}{91}                         & \percent[t]{1}{91}                      & \percent[t]{76}{91}                       & \percent[t]{5}{91}                          & \percent[t]{9}{91}                        \\
                        & Medium                      &   \percent[t]{23}{172}                   &  \percent[t]{99}{172}                      &  \percent[t]{23}{172}                      & \percent[t]{12}{172}                         & \percent[t]{15}{172}                        &   \percent[t]{26}{172}                   &  \percent[t]{119}{172}                     &  \percent[t]{13}{172}                      &  \percent[t]{10}{172}                        &  \percent[t]{4}{172}                        &   \percent[t]{31}{171}                   &     \percent[t]{105}{171}                   &     \percent[t]{19}{171}                      &   \percent[t]{16}{171}                       &  \percent[t]{29}{171}                    &  \percent[t]{116}{171}                     &  \percent[t]{17}{171}                        &  \percent[t]{9}{171}                       \\
                        & Easy                        &   \percent[t]{45}{88}                   &  \percent[t]{40}{88}                      &  \percent[t]{1}{88}                       &   \percent[t]{1}{88}                        &   \percent[t]{1}{88}                       & \percent[t]{45}{90}                     & \percent[t]{37}{90}                       & \percent[t]{4}{90}                        & \percent[t]{2}{90}                         & \percent[t]{2}{90}                         & \percent[t]{51}{89}                     & \percent[t]{31}{89}                       & \percent[t]{2}{89}                          & \percent[t]{5}{89}                         & \percent[t]{49}{89}                     &  \percent[t]{34}{89}                      & \percent[t]{1}{89}                          & \percent[t]{5}{89}                         \\ 
\cline{2-20}
                        & Total                       & \percent[t]{68}{351}                     & \percent[t]{196}{351}                      & \percent[t]{48}{351}                       & \percent[t]{20}{351}                         & \percent[t]{19}{351}                        & \percent[t]{71}{352}                     & \percent[t]{220}{352}                      & \percent[t]{33}{352}                       & \percent[t]{17}{352}                         & \percent[t]{11}{352}                        &  \percent[t]{84}{351}                    & \percent[t]{209}{351}                      & \percent[t]{32}{351}                         & \percent[t]{26}{351}                        & \percent[t]{79}{351}                     & \percent[t]{226}{351}                      & \percent[t]{23}{351}                         & \percent[t]{23}{351}                        \\ 
\midrule
\multirow{4}{*}{Bef.}   & Hard                        & \percent[t]{40}{94}                     & \percent[t]{18}{94}                       & \percent[t]{30}{94}                       & \percent[t]{2}{94}                          & \percent[t]{4}{94}                         & \percent[t]{47}{89}                     & \percent[t]{24}{89}                       & \percent[t]{12}{89}                       & \percent[t]{2}{89}                          & \percent[t]{4}{89}                         & \percent[t]{41}{90}                     & \percent[t]{30}{90}                       & \percent[t]{8}{90}                          & \percent[t]{11}{90}                        & \percent[t]{38}{90}                     & \percent[t]{42}{90}                       & \percent[t]{2}{90}                          & \percent[t]{8}{90}                         \\
                        & Medium                      & \percent[t]{125}{177}                    & \percent[t]{25}{177}                       & \percent[t]{21}{177}                       & \percent[t]{0}{177}                          & \percent[t]{6}{177}                         & \percent[t]{136}{174}                    & \percent[t]{21}{174}                       & \percent[t]{8}{174}                        & \percent[t]{6}{174}                          & \percent[t]{3}{174}                         &  \percent[t]{136}{172}                   & \percent[t]{28}{172}                       & \percent[t]{2}{172}                          & \percent[t]{6}{172}                         & \percent[t]{136}{169}                    & \percent[t]{22}{169}                       & \percent[t]{3}{169}                          & \percent[t]{8}{169}                        \\
                        & Easy                        & \percent[t]{91}{102}                     & \percent[t]{7}{102}                        & \percent[t]{2}{102}                        & \percent[t]{1}{102}                          & \percent[t]{1}{102}                         & \percent[t]{95}{101}                     & \percent[t]{4}{101}                        & \percent[t]{2}{101}                        & \percent[t]{0}{101}                          & \percent[t]{0}{101}                         & \percent[t]{95}{99}                     & \percent[t]{4}{99}                        & \percent[t]{0}{99}                          & \percent[t]{0}{99}                         & \percent[t]{94}{101}                     & \percent[t]{6}{101}                        & \percent[t]{0}{101}                          & \percent[t]{1}{101}                         \\ 
\cline{2-20}
                        & Total                       & \percent[t]{256}{373}                    & \percent[t]{50}{373}                       & \percent[t]{53}{373}                       & \percent[t]{3}{373}                          & \percent[t]{11}{373}                        & \percent[t]{278}{364}                    & \percent[t]{49}{364}                       & \percent[t]{22}{364}                       & \percent[t]{8}{364}                          & \percent[t]{7}{364}                         &  \percent[t]{272}{361}                   & \percent[t]{62}{361}                       & \percent[t]{10}{361}                          & \percent[t]{17}{361}                        & \percent[t]{268}{360}                    & \percent[t]{70}{360}                       & \percent[t]{5}{360}                          & \percent[t]{17}{360}                        \\ 
\midrule
-                       & Total                       & \percent[t]{324}{724}                    & \percent[t]{246}{724}                      & \percent[t]{101}{724}                      & \percent[t]{23}{724}                         & \percent[t]{30}{724}                        & \percent[t]{349}{716}                    & \percent[t]{269}{716}                      & \percent[t]{55}{716}                       & \percent[t]{25}{716}                         & \percent[t]{18}{716}                        & \percent[t]{356}{712}                    & \percent[t]{271}{712}                      & \percent[t]{42}{712}                         & \percent[t]{43}{712}                        & \percent[t]{347}{711}                    &  \percent[t]{296}{711}                     &  \percent[t]{28}{711}                        &   \percent[t]{40}{711}                      \\
\bottomrule
\end{tabular}}
\label{tab:generation-1}
\end{table*}



\begin{table}[ht]
\centering
\caption{Code-judged result in C language}
\renewcommand\arraystretch{1.3}
\scalebox{0.66}{\begin{tabular}{c|c|rrrrr} 
\toprule
\multirow{2}{*}{Period} & \multirow{2}{*}{Difficulty} & \multicolumn{5}{c}{C}             \\ 
\cline{3-7}
                        &                             & \multicolumn{1}{c}{A.}  & \multicolumn{1}{c}{W.A.} & \multicolumn{1}{c}{C.E.} & \multicolumn{1}{c}{T.L.E.} & \multicolumn{1}{c}{R.E.}  \\ 
\midrule
\multirow{4}{*}{Aft.}   & Hard                        & \percent[t]{0}{91}   & \percent[t]{57}{91}   & \percent[t]{25}{91}   & \percent[t]{2}{91}      & \percent[t]{7}{91}     \\
                        & Medium                      & \percent[t]{10}{170}  & \percent[t]{77}{170}   & \percent[t]{49}{170}   & \percent[t]{12}{170}     & \percent[t]{22}{170}    \\
                        & Easy                        & \percent[t]{44}{90}  & \percent[t]{33}{90}   & \percent[t]{9}{90}   & \percent[t]{0}{90}      & \percent[t]{4}{90}     \\ 
\cline{2-7}
                        & Total                       & \percent[t]{54}{351}  & \percent[t]{167}{351}  & \percent[t]{83}{351}   & \percent[t]{14}{351}     & \percent[t]{33}{351}    \\ 
\midrule
\multirow{4}{*}{Bef.}   & Hard                        & \percent[t]{17}{93}  & \percent[t]{36}{93}   & \percent[t]{31}{93}   & \percent[t]{3}{93}      & \percent[t]{6}{93}     \\
                        & Medium                      & \percent[t]{80}{172}  & \percent[t]{35}{172}   & \percent[t]{36}{172}   & \percent[t]{5}{172}      & \percent[t]{16}{172}    \\
                        & Easy                        & \percent[t]{74}{97}  & \percent[t]{9}{97}    & \percent[t]{6}{97}    & \percent[t]{0}{97}      & \percent[t]{8}{97}     \\ 
\cline{2-7}
                        & Total                       & \percent[t]{171}{362} & \percent[t]{80}{362}   & \percent[t]{73}{362}   & \percent[t]{8}{362}      & \percent[t]{30}{362}    \\ 
\midrule
-                       & Total                       & \percent[t]{223}{713} & \percent[t]{247}{713}  & \percent[t]{156}{713}  & \percent[t]{22}{713}     & \percent[t]{63}{713}    \\
\bottomrule
\end{tabular}}
\label{tab:generation-2}
\end{table}
